On The Potential of The Fractal Geometry and The CNNs Ability to Encode it

The fractal dimension provides a statistical index of object complexity by studying how the pattern changes with the measuring scale. Although useful in several classification tasks, the fractal dimension is under-explored in deep learning applications. In this work, we investigate the features that are learned by deep models and we study whether these deep networks are able to encode features as complex and high-level as the fractal dimensions. Specifically, we conduct a correlation analysis experiment to show that deep networks are not able to extract such a feature in none of their layers. We combine our analytical study with a human evaluation to investigate the differences between deep learning networks and models that operate on the fractal feature solely. Moreover, we show the effectiveness of fractal features in applications where the object structure is crucial for the classification task. We empirically show that training a shallow network on fractal features achieves performance comparable, even superior in specific cases, to that of deep networks trained on raw data while requiring less computational resources. Fractals improved the accuracy of the classification by 30% on average while requiring up to 84% less time to train. We couple our empirical study with a complexity analysis of the computational cost of extracting the proposed fractal features, and we study its limitation.

==> conclusion.tex <==
In this work, we inspected deep networks performance within the fractal geometry framework and we showed that DL models are unable to extract fractal features across different depth levels. We empirically demonstrate that shallow networks trained on the fractal features exhibit performance comparable to that of DL models that are trained on raw images while requiring less training time in specific tasks. In addition to that, given that fractal geometry studies the internal structure of complex objects, we reveal that such features can lead to better and more robust results in tasks where the study of the object substructure is crucial for classification. We also provide a theoretical complexity analysis showing that computing the fractal feature is efficient. We finally augment our study with a human evaluation of the wrong predictions by DL models as well as ZFrac+NN. The human evaluation showed that, on average, classifications missed by the fractal features are perceived as ``not obvious'' and harder to detect than those of DL models. A subsequent step in this line of work can focus on utilizing the fractal geometry in DL through architecture adaptation.  


